The rank 2 classification problem II: mapping scale-invariant solutions to SCFTs

This is the second of a series of papers outlining an approach to the classification of $\mathcal{N}{=}2$ superconformal field theories at rank 2 via a systematic analysis of their Coulomb branches, mathematically described by special K\"ahler scale invariant geometries. Here we describe how to make the translation between geometry and field theory data. We apply this strategy to the special K\"ahler geometries found in the first paper of the series where we made strong simplifying assumptions on the form of the solutions. Remarkably, we find that our bottom-up classification strategy pays off even in this simplified setup. All scale invariant solutions in the first paper of the series have an interpretation as the Coulomb branch of at least one $\mathcal{N}{=}2$ superconformal field theory, many matching what is already known. But we also predict the existence of six new rank 2 theories, including an entire new set closed under renormalization group flow. We characterise and discuss in detail each one of these new $\mathcal{N}{=}2$ superconformal field theories. To our knowledge none of them have known string theoretic or higher dimensional realisations.

==> Tables/CBDeltaR2.tex <==
\begin{table}[!t]
\begin{center}
\renewcommand{\arraystretch}{1.2}
\hspace*{-0.1cm}\begin{tabular}{c|c}
\multicolumn{2}{c}{\textsc{Genuinely rank-two pairs}}\\
\hline\hline
$P_i(z)$& $\{\D_1,\D_2\}$
\\\hline\hline
\multirow{2}{*}{$\Phi_5(z)$}&$\{\frac{4}{3},\frac53\}\ \{\frac54,\frac32\}\ \{\frac32,\frac52\}\ \{\frac54,3\}\ \{\frac53,3\}\ \{\frac52,3\}\ \{3,5\}\ \{\frac54,4\}$\\
&$\{\frac53,4\}\ \{\frac52,4\}\ \{4,5\}\ \{\frac54,8\}\ \{\frac53,8\}\ \{\frac52,8\}\ \{5,8\}$\\
\hline
\multirow{3}{*}{$\Phi_8(z)$}&$\{\frac65,\frac85\}\ \{\frac43,\frac83\}\ \{\frac87,\frac{10}7\}\ \{\frac87,\frac{12}7\}\ \{\frac85,\frac{12}5\}\ \{\frac83,\frac{10}3\}\ \{\frac87,4\}\ \{\frac85,4\}$\\
&$\{\frac83,4\}\ \{4,8\}\ \{\frac87,6\}\ \{\frac85,6\}\ \{\frac83,6\}\ \{6,8\}\ \{\frac87,12\}\ \{\frac85,12\}$\\
&$\{\frac83,12\}\ \{8,12\}$\\
\hline
\multirow{2}{*}{$\Phi_{10}(z)$}&$\{\frac{10}{9},\frac43\}\ \{\frac43,\frac{10}3\}\ \{\frac{10}9,4\}\ \{\frac{10}7,4\}\ \{\frac{10}3,4\}\ \{4,10\}\ \{\frac{10}9,8\}\ \{\frac{10}7,8\}$\\
&$\{\frac{10}3,8\}\ \{8,10\}$\\
\hline$\Phi_{12}(z)$&$\{\frac65,\frac{12}5\}\ \{\frac{12}{11},6\}\ \{\frac{12}7,6\}\ \{\frac{12}5,6\}\ \{6,12\}\ \{\frac{12}{11},8\}\ \{\frac{12}7,8\}\ \{\frac{12}5,8\}$\\
\hline\hline
\multicolumn{2}{c}{\textsc{Non-Genuine Rank-Two Pairs}}\\
\hline\hline
\multicolumn{2}{c}{$\{\D_1,\D_2\}$}\\
\hline\hline
\multicolumn{2}{c}{$\{\frac65,\frac65\}\ \{\frac65,\frac43\}\ \{\frac65,\frac32\}\ \{\frac65,2\}\ \{\frac65,3\}\ \{\frac65,4\}\ \{\frac65,6\}\ \{\frac43,\frac43\}\ \{\frac43,\frac32\}\ \{\frac43,2\}$}\\
\multicolumn{2}{c}{$\{\frac43,3\}\ \{\frac43,4\}\ \{\frac43,6\}\ \{\frac32,\frac32\}\ \{\frac32,2\}\ \{\frac32,3\}\ \{\frac32,4\}\ \{\frac32,6\}\ \{2,2\}\ \{2,3\}$}\\
\multicolumn{2}{c}{$\{2,4\}\ \{2,6\}\ \{3,3\}\ \{3,4\}\ \{3,6\}\ \{4,4\}\ \{4,6\}\ \{6,6\}$}\\
\hline\hline
\end{tabular}
\end{center}
\caption{Full list of allowed pairs of scaling dimensions at rank-two. The \emph{genuinely rank-two} pairs are those which include at least one entry which is not allowed at rank-one. In the first column we report the form of the characteristic polynomial where $\Phi_d(z)$ denotes a degree-$d$ cyclotomic polynomial. %At rank-two we should only consider those $d$ for which $\phi(d)=4$.
}
\label{tab:CBSDr2}
\end{table}%

==> Tables/CBDeltaR2_kappa.tex <==
\begin{table}[!t]
\begin{center}
\renewcommand{\arraystretch}{1.2}
\hspace*{-0.1cm}\begin{tabular}{c|c}
\multicolumn{2}{c}{\textsc{CB $\Delta$ with $\varkappa=\{1,2\}$}}\\
\hline\hline
& $\{\D_1,\D_2\}$
\\\hline\hline
\multirow{3}{*}{Polynomial Ansatz}&$\{\frac{10}{9},\frac43\}\ \{\frac87,\frac{12}7\}\ \{\frac65,\frac85\}\  \{\frac54,\frac32\}\ \{\frac{4}{3},\frac53\}\ \{\frac{4}{3},2\}\ \{\frac32,2\}\ \{\frac32,\frac52\}\  \{\frac53,3\}\  $\\
&$\{2,2\}\ \{2,3\}\ \{2,4\}\ \{\frac52,3\}\ \{\frac52,4\}\ \{\frac83,\frac{10}3\}\ \{\frac83,6\}\  \{3,4\}\  \{3,5\}\ $\\
&$\{\frac{10}3,4\}\ \{\frac{10}3,8\}\ \{4,5\}\  \{4,6\}\  \{4,10\}\ \{5,8\}\ \{6,8\}\ \{8,10\}  $\\
\hline
\multirow{3}{*}{Non-Polynomial}&$ \{\frac{10}9,4\}\  \{\frac{10}9,8\}\  \{\frac87,6\}\ \{\frac65,\frac43\}\  \{\frac65,2\}\ \{\frac65,4\}\  \{\frac54,3\}\ \{\frac54,4\}\ \{\frac54,8\}\ $\\
&$\{\frac43,\frac32\}\ \{\frac43,3\}\ \{\frac43,\frac{10}3\}\ \{\frac43,6\}\  \{\frac{10}7,4\}\  \{\frac{10}7,8\}\  \{\frac32,4\}\   \{\frac85,6\}\  $\\
&$\{\frac53,4\}\   \{\frac53,8\}\  \{2,6\}\  \{\frac52,8\}\  $\\
\hline\hline
\end{tabular}
\end{center}
\caption{Full list of allowed pairs of scaling dimensions at rank-two with characteristic dimension equal to one or two. These are further refined between those for which a hyperelliptic ansatz of the Seiber-Witten curve with polyonmial coefficients in $(u,v)$ is allowed and those for which it isn't.
}
\label{tab:CBSDr2kappa}
\end{table}%

==> Tables/unknown.tex <==

\begin{table}[ht]
\begin{adjustbox}{center,max width=.75\textwidth}
$\def\arraystretch{1.0}
\begin{array}{c:cc|c:cc|c:c:c:c}
\multicolumn{10}{c}{\Large \textsc{Rank-2\ theories\ with\ un-known\ hyperelliptic\ curve}}\\
\hline
\hline
\multicolumn{3}{l|}{\quad \text{Moduli Space}} &
\multicolumn{3}{l|}{\quad \text{Flavor and central charges}} &
\multicolumn{4}{c}{\quad \text{Curve information}}\\[1mm]
\D_{u,v}&\ \ d_{\text{HB}}\ \ &\ \  h\ \  
&\quad \ff\quad &\ \ 24a\ \ & 12c 
&\text{Dis}_{guess}&\text{Dis}_{real}&\text{form}&\text{partner}
\\[1.5mm]

%%%%%%%%%%%%%%%% [Sp(12) Sp(8) F4 series]

\cdashline{1-10}
\multicolumn{10}{c}{\spf(12)-\spf(8)-\ff_4\ \text{series}}\\
\hline
 \{4,6\} 
&  22 & 0
& \spf(12)_8 & 130 & 76  
&P_{knot}^2u^{12}&P_{knot}^2u^{12}& x^5 &\text{None}\\
 \{4,6\}
& 20 & 2
&\spf(4)_7 \times \spf(8)_8 & 128 & 74 
&P_{knot}u^8v^7&P_{knot}u^8v^{6}& x^6 &\text{None}\\
\{6,6\} 
&  24 & 2
& \suf(2)_7^2\times [\ff_4]_{12} & 156 & 90     
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
 \{3,4\}
&12 & 0
&\suf(2)_8\times \spf(8)_6 & 84  & 48 
&P_{knot}u^8v^{2}&P_{knot}u^8v^2& x^5 &\text{None} \\
 \{3,4\}
& 11 & 1
&\suf(2)_5\times \spf(6)_6\times \uf(1) & 83  & 47 
&P_{knot}u^6v^6&P_{knot}u^6v^5& x^6 &\text{None} \\
\{4,4\} 
& 12 & 2 
& \suf(2)_5^2\times \sof(7)_8 & 96 & 54    
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
 \{4,5\}
& 16 & 0
&[\ff_4]_{10}\times \uf(1) & 112  & 64
&P_{knot}v^8&P_{knot}v^8 & x^5 &\text{None} \\
 \{\frac52,3\}
&7 & 0
& \spf(6)_5\times \uf(1) & 61 & 34
&P_{knot}u^6&P_{knot}u^{6}& x^5 &\text{None} \\
 \{3,3\}
& 6 & 2
& \suf(3)_6\times\suf(2)^2_4 & 66 & 36  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
\rcy \{2,2\}
& 3 & 0
& \spf(4)_4 & 38 & 20 
&P_{knot}^4v^{4}&-& x^6 &\text{None}\\
\rcb \{2,2\}
&2 & 2
& \suf(2)_6 & 36 & 18    
&P_{knot}^6v^6&-& x^6 &\text{None}\\
\cdashline{1-10}

% SU(5) series


\multicolumn{10}{c}{\suf(5)\ \text{series}}\\
\hline

 \{6,8\}
& 19 & 0
&\suf(5)_{16} & 170 & 92  
&P_{knot}v^{8}&-& - &\text{None}\\
 \{4,6\}
& 6 & 0 &
\suf(3)_{12}{\times} \uf(1) & 114 & 60  
&P_{knot}u^2v^{6}&-& - &\text{None}\\
 \{3,5\}
& 3 & 0 &
\suf(2)_{10}{\times} \uf(1) & 86 & 44  
&P_{knot}v^*&-& - &\text{None}\\
\cdashline{1-10}



% Sp(12) series

\multicolumn{10}{c}{\spf(12)\ \text{series}}\\
\hline


 \{4,10\}
& 32 & 6
&\spf(12)_{11} & 188 & 110
&P_{knot}v^{11}&P_{knot}v^{10}& x^5 &\text{None}
\\
\rcy \{2,4\}
& 8 & 2
&\spf(4)_5 \times\sof(4)_8 & 68 & 38
&(P_{knot}^2)^2v^{7}&(P_{knot}^2)^2v^{6}& x^6 &\text{None}
\\
\rcy \{2,6\}
& 14 & 4
& \spf(8)_7 & 98 & 56
&P_{knot}^2v^{9}&P_{knot}^2v^{8}& x^6 &\text{None}
\\
 \{\frac43,\frac{10}3\}
& 4 & 2
& \spf(4)_{\frac{13}3} & 48 & 26
&P_{knot}v^{7}&P_{knot}v^{6}& x^6 &\text{None}
\\
 \{\frac32,\frac52\}
& 2 & 1
& \spf(2)_{7/2}\times\uf(1) & 38 & 20
&P_{knot}v^{6}&P_{knot}v^{5}& x^5 &\suf(5)_5
\\
[.5mm]

\cdashline{1-10}

% Sp(8) - SU(2)^2 series


\multicolumn{10}{c}{\spf(8)-\suf(2)^2\ \text{series}}\\
\hline
 \{6,12\}
& 28 & 6
& \spf(8)_{13}\times \suf(2)_{26} & 232 & 130  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
 \{4,8\}
& 14 & 4
& \spf(4)_{9}{\times} \suf(2)_{16} {\times}\suf(2)_{18}& 146 & 80  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
 \{3,6\}
&  7 & 3
& \suf(2)_{7}\times \suf(2)_{14}\times \uf(1) & 103 & 55  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
\{3,6\}   
& 6 & 2
& \suf(2)_6\times \suf(2)_8 & 102 & 54     
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
 \{\frac52,4\}
& 2 & 0
&\suf(2)_5 & 67 & 34 
&P_{knot} u^4&&&{\rm None}\\
\rcb \{2,4\}
&  2 & 
& \suf(2)_{10} & 60 & 30    
&\multicolumn{4}{c}{\rm Extended\ Automorphism?}\\
\cdashline{1-10}



% G2 series

\multicolumn{10}{c}{\gf_2\ \text{series}}\\
\hline
\{4,6\} 
& 12 & 2
& [\gf_2]_8\times \suf(2)_{14} & 120 & 66    
&P_{knot}^6 u^6&&&{\rm None}\\
\{\frac83,4\} 
& 4 & 2
& \suf(2)_{\frac{16}3}\times \suf(2)_{10}  & 72 & 38   
&\multicolumn{4}{c}{\rm Degenerate\ genus{-}2\ RS}\\
 \{\frac{10}3,4\}
& 6& 0
&[\gf_2]_{\frac{20}3} & 82  & 44
&P_{knot} u^6&&&{\rm None}\\
\rcb
\{2,3\}
& 2 & 2
& \suf(2)_8 & 48 & 24  
&\multicolumn{4}{c}{\rm Extended\ Automorphism}\\

\cdashline{1-10}

% SU(3) series

\multicolumn{10}{c}{\suf(3)\ \text{series}}\\
\hline

 \{6,12\}
& 15 & 5
& \suf(3)_{26}\times \uf(1) & 219 & 117  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
 \{4,8\}
& 5 & 3
& \uf(1)^2 & 137 & 71   
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
\rcg \{3,6\}
&  2 & 2
& \uf(1) & 96 & 48  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\

% SU(2) series

\cdashline{1-10}
\multicolumn{10}{c}{\suf(2)\ \text{series}}\\
\hline
 \{6,12\}
&  8 & 4
& \suf(2)_{16}\times \uf(1) & 212&  110  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\
\rcg \{4,8\}
&  2 & 2
& \uf(1) & 132 & 66  
&\multicolumn{4}{c}{{\rm Degenerate\ genus{-}2\ RS}}\\



\cdashline{1-10}


% Isolated theories

\multicolumn{10}{c}{\textsc{Isolated\ theories}}\\
\hline

 \{4,6\}
&  10 & 4
& \spf(4)_{14}\times\suf(2)_8 & 118 & 64   
&P_{knot}^7 u^2&&&{\rm None}\\
 \{\frac{12}5,6\}
&  2 & 2
& \suf(2)_{14} & \frac{456}5 & \frac{234}5   
&\multicolumn{4}{c}{\rm Degenerate\ genus{-}2\ RS}\\
\rcb \{2,6\}
& 2 & 2
& \suf(2)_{14} & 84 & 42    
&P_{knot}^7 u^2&&&{\rm None}\\
\rcy \{2,4\}
&  0 & 0
& \varnothing & 58 & 28  
&P_{knot}^5 v&&&{\rm None}\\


\hline\hline




%
\end{array}$
\caption{\label{tab:r21}%\footnotesize{List of rank-2 4$d$ theories with their corresponding CFT data and 5\emph{d} origin. The last column in the table gives the 5$d$ gauge theory description ofthe 5$d$ SCFT whose compactification gives the 4$d$ SCFT. Here we shallusually give only one gauge theory description although others mayexist. For most Lagrangian 4$d$ SCFTs, the 5$d$ parent is given by thecompactification of a 5$d$ gauge theory, rather than a 5$d$ SCFT. This isdenoted in the table by the label `GT'. When the compactification involves twisting, the discrete symmetry group being twisted is specified. In these cases this group is $\mathbb{Z}_2$ and it is manifested in the gauge theory as the combination of quiver reflection and charge conjugation. Notice that we use the convention $\spf(2n)$ where $n$ is rank. Also, compared to similar tables in \cite{Martone:2021ixp}, we won't report the SCFTs which can be obtained by mass-deforming the Lagrangian theories. Finally we shade in \yellow{yellow} $\cN=2$ Lagrangian theories and in \blue{blue} $\cN=4$ theories.}}
}
\end{adjustbox}
\end{table}
